Speech Wikimedia: A 77 Language Multilingual Speech Dataset

The Speech Wikimedia Dataset is a publicly available compilation of audio with transcriptions extracted from Wikimedia Commons. It includes 1780 hours (195 GB) of CC-BY-SA licensed transcribed speech from a diverse set of scenarios and speakers, in 77 different languages. Each audio file has one or more transcriptions in different languages, making this dataset suitable for training speech recognition, speech translation, and machine translation models.

==> tables/audio_durations.tex <==
\begin{table}[t]
\caption{Speech Recognition Task (No translation)}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Language & Duration (Hours) \\
\midrule
English (en) & 1965.577 \\
German (de) & 133.951 \\
Indonesian (id) & 102.961 \\
Turkish (tr) & 101.605 \\
Hindi (hi) & 100.499 \\
Dutch (nl) & 44.448 \\
Spanish (es) & 31.910 \\
Arabic (ar) & 25.179 \\
Portuguese (pt) & 15.742 \\
Russian (ru) & 12.120 \\
French (fr) & 9.245 \\
Polish (pl) & 7.887 \\
Ukrainian (uk) & 7.567 \\
Italian (it) & 7.112 \\
Norwegian (no) & 4.995 \\
Chinese (zh-cn) & 4.518 \\
Korean (ko) & 3.954 \\
Thai (th) & 3.234 \\
Swedish (sv) & 2.845 \\
Japanese (ja) & 2.494 \\
Bengali (bn) & 2.267 \\
Catalan (ca) & 2.145 \\
Czech (cs) & 1.984 \\
Nepali (ne) & 1.767 \\
Slovenian (sl) & 1.750 \\
Vietnamese (vi) & 1.500 \\
Greek (el) & 1.187 \\
Romanian (ro) & 1.172 \\
Hebrew (he) & 0.949 \\
Croatian (hr) & 0.937 \\
Welsh (cy) & 0.891 \\
Tagalog (tl) & 0.790 \\
Swahili (sw) & 0.777 \\
Macedonian (mk) & 0.712 \\
Finnish (fi) & 0.638 \\
Undetected (no\_detect) & 0.634 \\
Persian (fa) & 0.627 \\
Latvian (lv) & 0.617 \\
Hungarian (hu) & 0.612 \\
Estonian (et) & 0.378 \\
Somali (so) & 0.373 \\
Bulgarian (bg) & 0.306 \\
Chinese (zh-tw) & 0.280 \\
Danish (da) & 0.251 \\
Afrikaans (af) & 0.238 \\
Punjabi (pa) & 0.186 \\
Telugu (te) & 0.133 \\
Marathi (mr) & 0.106 \\
Urdu (ur) & 0.103 \\
Slovak (sk) & 0.101 \\
Tamil (ta) & 0.096 \\
Gujarati (gu) & 0.089 \\
Lithuanian (lt) & 0.074 \\
Kannada (kn) & 0.049 \\
Albanian (sq) & 0.032 \\
Malayalam (ml) & 0.022 \\
\hline
\bottomrule
\end{tabular}
\label{tab:total-time}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/language_duration_distribution.tex <==
\begin{table}[t]
\caption{Distribution of languages and their durations for transcriptions
X -> Y Speech Translation Task; Y is the language in column; X is unknown}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Language & Duration (Hours) \\
\midrule
English (en) & 2403.54 \\
Turkish (tr) & 315.94 \\
Korean (ko) & 315.69 \\
Czech (cs) & 206.55 \\
Spanish (es) & 193.38 \\
German (de) & 157.10 \\
Italian (it) & 127.44 \\
Indonesian (id) & 110.55 \\
Hindi (hi) & 101.79 \\
Dutch (nl) & 58.84 \\
Portuguese (pt) & 48.63 \\
French (fr) & 42.15 \\
Arabic (ar) & 41.27 \\
Russian (ru) & 37.29 \\
Estonian (et) & 19.07 \\
Polish (pl) & 17.41 \\
Chinese (Simplified) (zh-cn) & 16.65 \\
Ukrainian (uk) & 14.47 \\
Norwegian (no) & 10.23 \\
Vietnamese (vi) & 9.18 \\
Japanese (ja) & 9.12 \\
Swedish (sv) & 6.90 \\
Slovak (sk) & 6.36 \\
Catalan (ca) & 6.16 \\
Hebrew (he) & 5.52 \\
Greek (el) & 5.43 \\
Bulgarian (bg) & 5.34 \\
Thai (th) & 5.23 \\
Croatian (hr) & 5.09 \\
Hungarian (hu) & 4.74 \\
Latvian (lv) & 4.23 \\
Persian (fa) & 3.88 \\
Finnish (fi) & 3.64 \\
Bengali (bn) & 3.61 \\
Romanian (ro) & 3.52 \\
Slovenian (sl) & 3.30 \\
Macedonian (mk) & 2.90 \\
No Detection (no_detect) & 2.78 \\
Chinese (Traditional) (zh-tw) & 2.16 \\
Tagalog (tl) & 2.03 \\
Nepali (ne) & 1.94 \\
Welsh (cy) & 1.83 \\
Swahili (sw) & 1.56 \\
Danish (da) & 1.21 \\
Afrikaans (af) & 1.11 \\
Lithuanian (lt) & 0.94 \\
Somali (so) & 0.70 \\
Albanian (sq) & 0.57 \\
Punjabi (pa) & 0.44 \\
Telugu (te) & 0.40 \\
Tamil (ta) & 0.36 \\
Urdu (ur) & 0.26 \\
Malayalam (ml) & 0.21 \\
Marathi (mr) & 0.20 \\
Gujarati (gu) & 0.19 \\
Kannada (kn) & 0.17 \\
\hline
\bottomrule
\end{tabular}
\label{tab:total-time}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
